$\textbf{Only-IF}$:Revealing the Decisive Effect of Instruction Diversity on Generalization

Understanding and accurately following instructions is critical for large language models (LLMs) to be effective across diverse tasks. In this work, we rigorously examine the key factors that enable models to generalize to unseen instructions, providing insights to guide the collection of data for instruction-tuning. Through controlled experiments, inspired by the Turing-complete Markov algorithm, we demonstrate that such generalization $\textbf{only emerges}$ when training data is diversified enough across semantic domains. Our findings also reveal that merely diversifying within limited domains fails to ensure robust generalization. In contrast, cross-domain data diversification, even under constrained data budgets, significantly enhances a model's adaptability. We further extend our analysis to real-world scenarios, including fine-tuning of $\textit{$\textbf{specialist}$}$ and $\textit{$\textbf{generalist}$}$ models. In both cases, we demonstrate that 1) better performance can be achieved by increasing the diversity of an established dataset while keeping the data size constant, and 2) when scaling up the data, diversifying the semantics of instructions is more effective than simply increasing the quantity of similar data. Our research provides important insights for dataset collation, particularly when optimizing model performance by expanding training data for both specialist and generalist scenarios. We show that careful consideration of data diversification is key: training specialist models with data extending beyond their core domain leads to significant performance improvements, while generalist models benefit from diverse data mixtures that enhance their overall instruction-following capabilities across a wide range of applications. Our results highlight the critical role of strategic diversification and offer clear guidelines for improving data quality.

==> _intro.tex <==
\section{Introduction}
% The rapid advance of large language models (LLMs) is one of the most exciting recent developments in artificial intelligence. LLMs, pre-trained on large text corpora, have demonstrated impressive generalizable reasoning capabilities and can achieve remarkable performance across a broad set of tasks, ranging from natural language comprehension~\cite{wang2020superglue} and generation~\cite{brown2020language} to mathematical reasoning~\cite{cobbe2021gsm} and programming~\cite{chen2021codex}. These models have shown promise in performing real-world tasks in various applications and business solutions. While part of their success is attributed to their general reasoning abilities, the specific role of instruction following—the capability to interpret and act upon diverse prompts—remains less explored. Unlike complex reasoning and deduction, which often require deep contextual understanding, instruction following is about accurately capturing and adhering to the prompt's intentions.
The rapid advancements in large language models (LLMs) have revolutionized a wide range of tasks, including language comprehension~\citep{wang2020superglue}, generation~\citep{brown2020language}, knowledge-based question answering~\citep{hendrycks2021mmlu}, and solving complex reasoning problems in fields like mathematics~\citep{cobbe2021gsm,hendrycks2021math} and programming~\citep{chen2021humaneval,austin2021mbpp,chen2021codex,li2022alphacode}. These successes hinge on the foundational capabilities of LLMs, such as knowledge retrieval, reasoning, planning, and notably, instruction following—enabled through instruction-tuning~\citep{ouyang2022instructgpt,alpaca,wei2022flan,sanh2022t0}. Instruction-tuning trains LLMs on a wide variety of instruction-output pairs, allowing them to handle diverse prompts and better generalize to new tasks.

While knowledge retrieval focuses on accessing stored information and reasoning involves multi-step problem-solving, instruction following concerns the accurate interpretation and execution of diverse natural language prompts~\citep{zhou2023ifeval}. This capability is vital for user interaction, as it involves understanding the intent behind instructions and performing tasks without relying on complex logic~\citep{liu2024incompleteloopinstructioninference}. Despite its importance, the mechanisms underlying instruction following remain less explored compared to other capabilities like reasoning.

The current research landscape on instruction tuning has produced varied and sometimes contradictory findings, ranging from the impact of dataset selection~\citep{zhou2023lima} to the effects of scaling up data~\citep{zeng2024skyworkmathdatascalinglaws,zhang2024scale}. These disparate findings suggest that instruction following in LLMs is influenced by the scale and composition of fine-tuning data in complex ways~\citep{dong2024composition,zhang2024unveilingimpactcodingdata}. However, a systematic investigation into the effect of data on each core capability of LLMs —specifically isolating instruction following from reasoning and knowledge retrieval—has been limited. As a result, there is a lack in principled and practical guidelines on how to compose data to improve instruction-following capabilities.

Our work addresses this gap by focusing explicitly \textbf{ONLY} on the \textbf{I}nstruction-\textbf{F}ollowing capabilities of LLMs. We first introduce a systematic analysis of instruction diversity through a controlled symbolic task—string rewrites—inspired by the Turing-complete Markov algorithm~\cite{markov54}. By isolating the effects of instruction diversity, we focus on the model's ability to follow instructions without conflating this with reasoning capabilities. 
Through controlled experiments, we examine the impact of instruction diversification across various semantic domains on the model's ability to adapt to unseen instruction semantics. We find that generalization to unseen task semantics emerges \textbf{ONLY IF} the instructions are sufficiently diversified. Our findings reveal that diversification confined to limited domains does not guarantee robust generalization. In contrast, cross-domain diversification significantly enhances the model's adaptability to new instructions, highlighting the importance of a more diverse training strategy.
\begin{figure}[ht]
     \centering
     \begin{subfigure}[h]{.3\textwidth}
     \centering
         \includegraphics[width=\columnwidth]{assets/multi+cot.pdf}
         \caption{\small Semantic clustering of relevant datasets.}
         \label{fig:emb-all}
     \end{subfigure}
     \hfill
     \centering
     \begin{subfigure}[h]{.3\textwidth}
     \centering
         \includegraphics[width=\columnwidth]{assets/temp_20000.pdf}
         \caption{\small OSS-Alpaca mixture and test instructions.}
         \label{fig:emb-train}
     \end{subfigure}
     \hfill
     \centering
     \begin{subfigure}[h]{.3\textwidth}
     \centering
         \includegraphics[width=\columnwidth]{assets/oss_cot_alpaca_2000_only.pdf}
         \caption{OSS-COT-Alpaca mixture and test instructions.}
         \label{fig:emb-train-cot}
     \end{subfigure}
     \caption{\small Visualization of embedded instructions.}
\end{figure}


% We extend our analysis to real-world LLM fine-tuning tasks, considering two scenarios: fine-tuning for \textbf{specialist} LLMs (e.g., training a programming-specific LM) and \textbf{generalist} LLMs (handling various tasks). Through training Code-LMs, we show that balancing specialization and generalization in data improves the \textbf{specialist} model's instruction-following abilities and accuracy. In the \textbf{generalist} scenario, diversifying instruction domains significantly enhances the model's capability to follow instructions from domains it has not been trained on, thus boosting the overall capability.
Additionally, our research offers and empirically verifies key insights into dataset collation strategies for both \textbf{specialist} and \textbf{generalist} LLMs. We show that when training \textbf{specialist} models (e.g., code language models), extending data diversification beyond their core domain yields substantial performance improvements in instruction following. For \textbf{generalist} models, using diverse data mixtures enhances their instruction-following capabilities across a broad range of applications, even for domains they were not explicitly trained on. 

For both \textbf{specialist} and \textbf{generalist} models, we showed that our findings can imply 1) better performance than training on established datasets can be achieved by increasing the dataset's diversity while maintaining the same data size, and 2) when scaling up the data, diversifying instruction semantics is more effective than simply increasing the amount of data from the same distribution.

These findings emphasize the importance of diversification in optimizing LLM performance and adaptability. Our study provides insights for dataset collation, especially when \textit{\textbf{dataset expansion}} is needed, showing how proper data diversification boosts performance in both specialist and generalist LLM scenarios, and is more effective than even multiplying dataset sizes.

The rest of the paper is organised as follows:

We introduce the Markov-algorithm style rewrite experiments and our findings in Section~\ref{sec:markov_section2}. In Section~\ref{sec:rewrite_with_abstraction_sec3} we generalize the rewriting by introducing abstraction, to simulate the situation of specialist and generalist training. In Section~\ref{sec:specialist_sec4} we 


% Specifically, we demonstrate that cross-domain instruction diversity is crucial for generalizing instruction-following capabilities in contexts such as code generation and general reasoning tasks. This cross-domain approach enables LLMs to handle previously unseen instructions more effectively. 

% \chihan{Hao dropped my ``contribution'' paragraph before}
% Our key contributions are summarized as follows:
% \begin{itemize}
%     \item We introduce a symbolic string rewrite task to systematically isolate and analyze instruction-following, offering a new lens on this crucial capability.
%     \item We systematically demonstrated the importance of instruction diversity within a fixed data budget as a \textbf{decisive factor} to generalization. 
%     \item We provide insights for dataset collation, especially when \textit{\textbf{dataset expansion}} is needed, showing how proper data diversification boosts performance in both specialist and generalist LLM scenarios, and is more effective than even multiplying dataset sizes. 
% \end{itemize}
% \begin{itemize}
%     \item We establish that instruction diversity is essential for enhancing generalization, allowing models to comprehend and execute previously unseen instruction semantics.
%     \item We identify cross-domain instruction diversity as the most effective strategy for developing a language model 
%     \item By providing a systematic exploration of cross-domain diversity, we offer new insights into instruction tuning for LLMs. These findings contribute to a better understanding of LLM versatility and applicability, complementing existing research on complex reasoning.
% \end{itemize}







% By examining how LLMs can be optimized for interpreting and responding to diverse prompts, we seek to provide a clearer understanding of the principles that guide effective instruction following.

% Works like InstructGPT~\citep{ouyang2022instructgpt}, FLAN~\citep{wei2022flan}, and T0~\citep{sanh2022t0} have demonstrated that fine-tuning on a collection of instructions can significantly improve a model's ability to follow unseen prompts. 
% It is generally believed that instruction diversity is crucial for enabling LLMs to generalize to unseen tasks. Several studies have acknowledged this by constructing large, diverse instruction datasets, such as NaturalInstructions and P3. These efforts have indeed shown that a variety of tasks can improve instruction-following performance. However, they fall short in conclusively demonstrating that instruction diversity is the enabling factor for a model's ability to understand and execute unseen instruction semantics. Existing works primarily focus on dataset construction rather than systematically analyzing the direct impact of cross-domain instruction diversity on adaptability and generalization.



% \emph{Instruction tuning} is a popular approach to unlock the capabilities of these models originally trained on next-token-prediction objectives to understand instructions and perform reasoning to complete tasks. By training models on pairs of instructions and expected outcomes, instruction tuning teaches LLMs to perform specific tasks, thus enabling them to address real-world problems and seamlessly interact with humans. In practice, however, fine-tuning data is limited, and instruction tuning can only focus on a limited set of tasks. Its success is therefore critically dependent on the model's ability to generalize beyond its fine-tuning instructions to \emph{unseen tasks} not encountered during training. Several factors influence this generalization: the size of the fine-tuning sample, the diversity of the instruction sets, and the quality of the annotations. Yet, there is little systematic research on their relative impact.

% Our work aims to fill this gap by proposing \textbf{two contributions} to the study of generalization in instruction tuning. First, we propose a systematic analysis of the \textbf{impact of instruction diversity} by focusing on a simple yet important symbolic task: \textbf{string rewrites}. This basic setting enables us to exercise fine control over the factors that may affect generalization and to demonstrate the importance of instruction diversity. To highlight the broader applicability, we describe this task in terms of a Markov algorithm, a classic Turing-complete model, ensuring rigorous examination of string replacements. Second, we extend this analysis to \textbf{a real-world application: code generation}, and show that fine-tuning on an instruction set that extends beyond coding tasks significantly improves performance.

% Our \textbf{main findings} are:
% \begin{enumerate}[nosep]
% \item Instruction diversity is the main driver of generalization. Models trained on a diverse set of instructions generalize better, even when the number of examples per instruction is small.
% \item The semantic diversity of instructions matters, together with the number of instructions.
% \item Instruction diversity improves model robustness and can compensate for the adverse impact of non-uniform fine-tuning distributions.
% \end{enumerate}

% We demonstrate that generalization and robustness with respect to the training distribution emerge once a diverse enough set of tasks is provided, even though very few examples are provided for each task. These initial results are extended to a real-world application scenario of code generation, where we find that a more diverse instruction set, extending beyond code-related tasks, improves performance. Our observations suggest that a more diverse semantic space for instruction-tuning sets greatly improves the model's ability to follow instructions and perform tasks. 
